DISCO: DISCovering Overfittings as Causal Rules for Text Classification Models

With the rapid advancement of neural language models, the deployment of over-parameterized models has surged, increasing the need for interpretable explanations comprehensible to human inspectors. Existing post-hoc interpretability methods, which often focus on unigram features of single input textual instances, fail to capture the models' decision-making process fully. Additionally, many methods do not differentiate between decisions based on spurious correlations and those based on a holistic understanding of the input. Our paper introduces DISCO, a novel method for discovering global, rule-based explanations by identifying causal n-gram associations with model predictions. This method employs a scalable sequence mining technique to extract relevant text spans from training data, associate them with model predictions, and conduct causality checks to distill robust rules that elucidate model behavior. These rules expose potential overfitting and provide insights into misleading feature combinations. We validate DISCO through extensive testing, demonstrating its superiority over existing methods in offering comprehensive insights into complex model behaviors. Our approach successfully identifies all shortcuts manually introduced into the training data (100% detection rate on the MultiRC dataset), resulting in an 18.8% regression in model performance -- a capability unmatched by any other method. Furthermore, DISCO supports interactive explanations, enabling human inspectors to distinguish spurious causes in the rule-based output. This alleviates the burden of abundant instance-wise explanations and helps assess the model's risk when encountering out-of-distribution (OOD) data.

==> 03-approach-post-ecai.tex <==
\section{Causal Rule Mining}
\label{sec:approach}
\subsection{Problem Statement}
We consider an underlying model $M$ trained on a classification dataset represented as $\mathcal{D} \subset \mathcal{X} \times \mathcal{Y}$.
Here, $\mathcal{X}$ represents the input space, and $\mathcal{Y}$ represents the labels.
An input $\mathbf{x} \in \mathcal{X}$ is an ordered sequence of terms $(x_1, x_2, \ldots, x_{|\mathbf{x}|})$, where each term $x_i$ comes from the vocabulary $\mathcal{V}$.
The prediction made by $M$ on input $\mathbf{x}$ is denoted as $\hat{y} = \text{argmax}_{y \in \mathcal{Y}} P_{M}(y|\mathbf{x})$.
For simplicity, we abbreviate this as $\hat{y} = M(\mathbf{x})$ throughout this paper.
Our research focuses exclusively on binary classification tasks.

We define $\mathbf{s} = (s_1, s_2, \dots, s_n)$ as an n-gram sub-sequence of $\mathbf{x}$ (represented as $\mathbf{s} \sqsubseteq \mathbf{x}$).
The remaining content in $\mathbf{x}$ is denoted as $\mathbf{c}$, i.e., $\mathbf{x} = \langle \mathbf{s}, \mathbf{c} \rangle$, where $\langle \cdot, \cdot \rangle$ is the sequence combination operator.
Note that we do not assume sequence continuity in either $\mathbf{c}$ or $\mathbf{s}$.
The support of $\mathbf{s}$ within $\mathcal{D}$ is defined as $\operatorname{Sup}(\mathbf{s}, \mathcal{D}) = |\left\{\mathbf{x} \in \mathcal{D} : \mathbf{s} \sqsubseteq \mathbf{x}\right\}|$.

Additionally, we define a rule $r$ as a tuple $(\mathbf{s} \rightarrow \hat{y})$, where the sequence $\mathbf{s}$ is its \textit{pattern} and $\hat{y}$ is its \textit{consequent} label.
For instance, the rule:
\begin{equation*}
\underbrace{\mathtt{\underline{the\, best \,movie}}}_{\text{\textit{pattern}}} \rightarrow \underbrace{\mathtt{\texttt{POS}}}_{\text{\textit{consequent}}}
\end{equation*}
indicates that ``\underline{the best movie}'' is a shortcut for $M$ to predict \textbf{POS}itive.
In this context, we say that $\mathbf{s}$ causes $M$ to predict $\hat{y}$, rather than that the $M$ comprehends the overall input $\mathbf{x}$.
% In this context, we say that $M$ predicts $\hat{y}$ primarily relying on the presence of the sequence $\mathbf{s}$, rather than comprehending the overall input.

Our objective is to discover a globally representative set of rules, denoted as $G = \{r = (\mathbf{s}, \hat{y})\}$, where each rule is a shortcut.

\subsection{DISCO: Approach Overview}
\label{sec:overview}
We divide our approach into two phases, i.e. the traditional statistic phase (Section~\ref{sec:sequence-mining}) and the causal inference phase (Section~\ref{sec:causality_check}).
In the first phase, we extract all high-frequency n-gram patterns from the training data and only keep such sequences, which again frequently co-occurs with a specific model prediction (Section~\ref{sec:sequence-mining}).
In the second phase, we apply a straightforward causal inference verification referred as the ``causality check'' (Section~\ref{sec:causality_check}) to the co-occurring sequence and model prediction.
The causality check identifies whether they are statistically correlated or do the sequences cause biased predictions.

\subsection{Generation of Candidate Sequences}
\textbf{Sequence Mining.}
\label{sec:sequence-mining}
Empirical studies such as~\cite{idahl-etal-2021-decoy} emphasize that a pattern is more likely to influence a model's prediction as a shortcut if it occurs frequently in the training set.
Therefore, we start from mining all frequent patterns.
The sequence-mining is a well-researched problem with a plenty of approaches.
Specifically, in \approach{}, we use an efficient approach, DESQ-COUNT~\cite{beedkar2019desq} to mine all frequent sequences from the training data.
For a detailed explanation of DESQ-COUNT, we refer to~\cite{Beedkar_Gemulla_Martens_2019}.

\textbf{NPMI Evaluation.}
\label{sec:npmi}
We further evaluate the NPMI (Normalized Pointwise Mutual Information) score between the pattern and each model prediction correlation and keep all sequences showing much higher NPMI with one label than the other.
For all input data $\mathbf{x}$ containing an $\mathbf{s}$ and their model predictions $\hat{y} = M(\mathbf{x})$, we can easily calculate $P(y, \mathbf{s})$, $P(y|\mathbf{s})$, and $P(y)$.
It is worth mentioning that these probabilities are different from the $P_M(\hat{y}|\mathbf{x})$ as the model's prediction.
The NPMI scores for an $\mathbf{s}$ regarding $\mathbf{y}$ is calculated as follows:
\begin{equation*}
\text{NPMI}(\mathbf{s}; y) = \frac{\text{PMI}(y ; \mathbf{s})}{h(\mathbf{s}, y)} = \frac{\log \frac{P(y|\mathbf{s})}{P(y)}}{h(\mathbf{s}, y)},
\end{equation*}
where $h(\mathbf{s}, y) = -\log P(\mathbf{s}, y)$ is the entropy of $P(\mathbf{s}, y)$.
The NPMI score falls within the range of $[-1, 1]$, capturing the spectrum from ``never occurring together (-1)'' to ``independence (0)'' and ultimately ``complete co-occurrence (1)'' between the pattern and the label.
We retain only those pairs that demonstrate a substantial level of correlation in their NPMI scores.

\subsection{Causality Check}
\label{sec:causality}
\label{sec:causality_check}
Such correlation alone, however, does not indicate a causal relationship, as it could also arise from a confounding variable~\cite{pearl2009causality}.
In order to define and figure out the confounding variable, we construct a Structured Causal Model (SCM)~\cite{pearl2009causality} to describe the prediction process of a non-overfitting classifier, as illustrated in Figure ~\ref{fig:graph_models}.
Here, we assume the confounding variable as the latent semantic representation $\mathbf{z}$ of the input, and the selection of sequence pattern $\mathbf{s}$ and the context $\mathbf{c}$ is conditioned on $\mathbf{z}$.
The input $\mathbf{x}$ depends depends on both $\mathbf{s}$ and $\mathbf{c}$ deterministically, and the model $M$ predicts $\hat{\mathbf{y}}$ given $\mathbf{x}$.
Ideally, a classifier predicts based on this decision model and therefore comprehends $\mathbf{z}$.
If a classifier predicts merely relying on the statistical correlation between $\mathbf{s}$ and $\hat{y}$, or ``there is causal relationship between $\mathbf{s}$ and $\hat{y}$'' using the language of causal inference, $\mathbf{z}$ no longer serves as the confounding variable of the correlation.
Reflected on the SCM, this indicates the connection from the $\mathbf{z}$ and $\mathbf{s}$ is broken.
In this case, $M$ is considered making a ``shortcut'' prediction based on $\mathbf{s}$~\cite{jacobsen2020shortcuts, Bastings2021shortcuts}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/graph_model_confounding_v2.pdf}
    \label{fig:graph_conf}
    \caption{The SCM describing the prediction process of an ideal model.
    Capital letters represent corresponding random variables.}
    \label{fig:graph_models}
\end{figure}

Following~\cite{pearl2009causality}, we apply the \textbf{do-operator} on the variable $\mathbf{s}$ to determine the causal relationship between $\mathbf{s}$ and $\hat{y}$.
The do-operator simulates a physical intervention by replacing a random variable (RV) with a constant value while keeping the rest of the RVs intact, thereby breaking the potential confounding effect.
In our SCM, applying the do-operator to $\mathbf{s}$ means assigning $\mathbf{s}$ a specific value and marginalizing over context $\mathbf{c}$.

If the $\mathbf{s}$ -- $\hat{y}$ correlation is caused by the confounding factor $\mathbf{z}$ (ideal classifier), the prediction of $M$ should differ before and after applying the do-operator, while an overfitting classifier shows no such difference: 
\begin{align*}
P(\hat{y}|\mathbf{s}) 
&= \sum_{z, \mathbf{c}}P(\hat{y}|\mathbf{s}, \mathbf{c})P(\mathbf{c}, \mathbf{s}|z)P(z) \\
&\neq  \sum_{z, \mathbf{c}}P^*(\hat{y}|\mathbf{s}, \mathbf{c})P^*(\mathbf{c}|z)P^*(z) 
= P(\hat{y}|\text{do}(\mathbf{s}=\mathbf{s})),
\end{align*}
where $P^*(\cdot)$ denotes the distributions after applying the do-operator.

Despite the similarity between \approach{} and that in~\cite{Wang_Culotta_2020}, their work distinguishes between ``spurious'' and ``genuine'' local shortcuts based on human understanding.
Rules produced by our approach possess a causal attribute globally without targeting such distinction due to subjectivity concerns.
To highlight the difference between semantically spurious (that in~\cite{Wang_Culotta_2020}) and causal shortcuts (ours), we measure human agreement on distinguishing ``right'' from ``wrong'' shortcuts in Section~\ref{sec:human-eval}.

\textbf{Neutral Context Harvesting.}
\label{sec:neutrality}
One remaining challenge in the algorithm mentioned in the previous section is sampling the context RV $\mathbf{C}$.
We employ a straightforward technique to extract neutral context by reusing contexts $\mathbf{c}$ for different $\mathbf{s}$, effectively obtaining contexts for free.
A context is neutral when its results in model's prediction lying near the border between two labels, namely $|P_M(y=y_0|\mathbf{c}) - P_M(y=y_1|\mathbf{c})| = |2P_M(y=y_0|\mathbf{c}) - 1| < \epsilon_n$, where $0 < \epsilon_n < 1$ is the neutrality tolerance.
We use the neutral contexts only, instead of reuse all context, to mitigate the influence of other potential frequent sequences might existing in the context.
Complex modern numerical sampling techniques, such as Markov Chain Monte Carlo (MCMC) \cite{metropolis1953equation}, require careful handling to preserve contextual fluency and ensure the neutrality of the sentiment.
Therefore, perfecting the generation of bias-free and neutral counterfactual contexts is left for future works.

\subsection{A Toy Example}
At the end of this section, we provide a toy example to assist our readers in understanding the full process of our approach.
We consider an extreme biasing sentiment analysis dataset, where all reviews on \textbf{books} are \textbf{positive}, and all reviews on \textbf{movies} are \textbf{negative} in the training data.
A model trained on such data might incorrectly predict \textbf{positive} for a review like ``this book is badly written'' due to the shortcut ``this book'' $\rightarrow$ \textbf{positive}.
Although such sequences may appear semantically senseless and non-causal to humans, the resulting rules reflect rationale of the model.

We at first identify the frequent, high-correlating sequence ``this book'' and its label \textbf{positive} from the training data (Section~\ref{sec:sequence-mining}).
Then, we keep ``this book'' constant and vary its contexts to other neutral contexts like ``was played in the cinema'' or ``is on the table'' (Section~\ref{sec:causality}).
If the prediction predominantly remains \textbf{positive}, ``this book'' $\rightarrow$ \textbf{positive} is a shortcut rule.


==> algorithm.tex <==
% \begin{algorithm}[t]
%     \DontPrintSemicolon
%     \SetKw{Yield}{Yield}
%     \SetKwInOut{Require}{Require}
%     \Require{the set of all inputs $\mathcal{X}$, all candidate sequences passing the \textcolor{red}{NPMI check} $\mathbf{S}$ and their correlated labels $\mathbf{\hat{Y}}$}
%     $C \gets \{\}$ \;
%     \ForAll{$\mathbf{s} \in \mathbf{S}$}{
%         $C \cap = \{\mathbf{c} = (\mathbf{p}, \mathbf{q}) |\mathbf{x} = <\mathbf{p}, \mathbf{s}, \mathbf{q}> \in \mathcal{X} \}$\;
%         \tcp{Retrieve contexts}
%     }
%     $\mathbf{C}^n$ := $\{\mathbf{c}|\mathbf{c} \in \mathbf{C} \text{ is neutral w.r.t. }M\}$\;
%     \tcp{Neutrality check, see \textcolor{red}{4.6}}
%     \ForAll{$(\mathbf{s}, \hat{y})\in \text{zip}(\mathbf{S}, \hat{Y})$}{
%         $\text{Syn}_\mathbf{s} \gets \{\}$\;
%         \ForAll{$\mathbf{c}' = (\mathbf{p}',\mathbf{q}')\in \mathbf{C}^n$}{
%             $\text{Syn}_\mathbf{s} += <\mathbf{p}', \mathbf{s}, \mathbf{q}'>$\;
%             \tcp{Synthesize inputs}
%         }
%         $\bar{y}_\mathbf{s} = \text{argmax}_{\bar{y}\in\mathcal{Y}}\frac{1}{|\text{Syn}_\mathbf{s}|}\sum_{\mathbf{x}' \in \text{Syn}_\mathbf{s}}P_M(y=\bar{y}|\mathbf{x}')$\;
%         \uIf{$\bar{y}_\mathbf{s} = \hat{y}$}{
%             \Yield "Causal Rule: $\mathbf{s}\to \hat{y}$"\;
%         }
%         \Else{
%             \Yield "No causal relationship between $\mathbf{s}$ and $\hat{y}$"\;
%         }
%     }
%     \caption{Causality Check}
%     \label{alg:causality}
% \end{algorithm}


% \begin{algorithm}[H]
%     \DontPrintSemicolon
%     \SetKwFunction{Sparse}{sparse}
%     \SetKwFunction{Max}{max}
%     \SetKw{In}{in}
%     \SetKw{Break}{break}
%     \KwIn{query $q$, sparse retrieval depth $k_S$, cut-off depth $k$, interpolation parameter $\alpha$}
%     \KwOut{approximated top-$k$ scores $Q$}
%     $Q \leftarrow$ priority queue of size $k$\;
%     $s_{D} \leftarrow -\infty$\;
%     $s_{min} \leftarrow -\infty$\;
%     \ForEach{$d$ \In $\Sparse(q, k_S)$}{
%         \uIf{$Q$ is full}{
%             $s_{min} \leftarrow$ remove smallest item from Q\;
%             $s_{best} \leftarrow \alpha \cdot \phi_S(q, d) + (1 - \alpha) \cdot s_{D}$\; \label{alg:early_stopping:sbest}
            
%             \uIf{$s_{best} \leq s_{min}$}{
%                 \tcp{early stopping}
%                 put $s_{min}$ into $Q$\;
%                 \Break\;
%             }
%         }
%         \tcp{approximate max. dense score}
%         $s_{D} \leftarrow \Max(\phi_D(q, d), s_{D})$\;
%         $s \leftarrow \alpha \cdot \phi_S(q, d) + (1 - \alpha) \cdot \phi_D(q, d)$\;
%         put $\Max(s, s_{min})$ into $Q$\;
%     }
%     \Return{$Q$}\;
%     \caption{Interpolation with early stopping}
%     \label{alg:early_stopping}
% \end{algorithm}

==> tables/rq1-agreement.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|l|l|l|l|}
        \hline
        dataset                 & rule & cov & agg$L$ & agg$^E$ \\
        \hline
        \multirow{3}{*}{\movies} 
            & \textit{one of the worst} $\to$ \textbf{NEG}  & .957 & .676 & .916\\
            & \textit{there ' s nothing} $\to$ \textbf{NEG} & .857 & .736 & .918\\
            & \textit{don ' t even} $\to$ \textbf{NEG}      & .826 & .742 & .914\\
        \hline
        \multirow{3}{*}{\multirc} 
            & (\textit{? | |}, \textit{, according to a}) $\to$ \textbf{False}          & .722 & (-, .831) & (.835, .906)\\
            & (\textit{? | |}, \textit{of the world trade center}) $\to$ \textbf{False} & .706 & (-, .770) & (.850, .912) \\
            & (\textit{? | |}, \textit{to get to the}) $\to$ \textbf{False}             & .667 & (-, .849) & (.814, .894)\\
        \hline
        \multirow{3}{*}{\sst} 
            & \textit{the best} $\to$ \textbf{POS} & .872 & .727 & .867\\
            & \textit{a good} $\to$ \textbf{POS}   & .704 & .800 & .849\\
            & \textit{in its} $\to$ \textbf{POS}   & .643 & .822 & .830\\
        \hline
        \multirow{3}{*}{\climate} 
            & (\textit{global warming}, \textit{climate system}) $\to$ \textbf{relevant}          & 1.0 & - & (.852, .932)\\
            & (\textit{global warming}, \textit{intergovernmental panel}) $\to$ \textbf{relevant} & 1.0 & - & (.849, .924)\\
            & (\textit{global warming}, \textit{the earth}) $\to$ \textbf{relevant}               & 1.0 & - & (.848, .922)\\
        \hline
    \end{tabular}
    \caption{Averaged rank scores over supporting instances of the rules with top coverage (cov). The agg$^{\{E, L\}}$ indicates the local agreement score of the global rule with respect to the local explanation produced by \expred~($E$) and \lime~($L$). \textcolor{red}{this table will be replaced by table \ref{tab:human_evaluation}}}
    \label{tab:faithful}
\end{table*}


\begin{table*}[h]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
        \hline
        dataset                 & rule & cov & MRR$^E$ & MAP$^E$ & nDCG$^E$ & MRR$^L$ & MAP$^L$ & nDCG$^L$\\
        \hline
        \multirow{3}{*}{\movies} & one of the worst $\to$ NEG & .957 & .262 & .240 & .676 & .092 & .041 & .916\\
        & there ' s nothing $\to$ NEG & .857 & .032 & .045 &	.736 & .098 & .035 & .918\\
        & don ' t even $\to$ NEG & .826 & .021 & .034 & .742 & .055 & .025 & .914\\
        \hline
        \multirow{3}{*}{\multirc} 
        & ? | | [SEP] , according to a $\to$ NEG & .722 & .078|.018 & .140|.033 & 0.0|.831 & .506|.043 & .441|.024 & .835|.906\\
        & ? | | [SEP] of the world trade center $\to$ NEG & .706 & .074|.054 & .134|.041 & 0.0|.770 & .635|.070 & .416|.031 & .850|.912 \\
        & ? | | [SEP] to get to the $\to$ NEG & .667 & .108|.015 & .190|.030 & 0.0|.849 & .500|.030 & .418|.024 & .814|.894\\
        \hline
        \multirow{3}{*}{\sst} 
        & the best $\to$ POS & .872 & .194 & .201 & .727 & .541 & .393 & .867\\
        & a good $\to$ POS & .704 & .275 & .264 & .800 & .506 & .345 & .849\\
        & in its $\to$ POS & .643 & .248 & .222 & .822 & .225 & .186 & .830\\
        \hline
        \multirow{3}{*}{\climate} 
        & global warming [SEP] climate system $\to$ relevant & 1.0 & -& -& -& .287|.035 & .240|.024 & .852|.932\\
        & global warming [SEP] intergovernmental panel $\to$ relevant & 1.0 & - & - & - & .278|.042 & .242|.029 & .849|.924\\
        & global warming [SEP] the earth $\to$ relevant & 1.0 & - & - & - & .285|.038 & .246|.027 & .848|.922\\
        \hline
    \end{tabular}
    \caption{Averaged rank scores over supporting instances of the rules with top coverage (cov). the scores with the superscript $^E$ are scores with \expred, while $^S$ indicates \lime. \textbf{Do the global rules agree with the local explanations of their applicable instances'?}}
    \label{tab:faithful}
\end{table*}




% \begin{table*}[h]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
%         \hline
%         dataset                 & rule & cov & MRR$^E$ & MAP$^E$ & nDCG$^E$ & MRR$^L$ & MAP$^L$ & nDCG$^L$\\
%         \hline
%         \multirow{3}{*}{\movies} & one of the worst $\to$ NEG & .957 & .262 & .240 & .676 & .092 & .041 & .916\\
%         & there ' s nothing $\to$ NEG & .857 & .032 & .045 &	.736 & .098 & .035 & .918\\
%         & don ' t even $\to$ NEG & .826 & .021 & .034 & .742 & .055 & .025 & .914\\
%         \hline
%         \multirow{3}{*}{\multirc} 
%         & ? | | [SEP] , according to a $\to$ NEG & .722 & .078|.018 & .140|.033 & 0.0|.831 & .506|.043 & .441|.024 & .835|.906\\
%         & ? | | [SEP] of the world trade center $\to$ NEG & .706 & .074|.054 & .134|.041 & 0.0|.770 & .635|.070 & .416|.031 & .850|.912 \\
%         & ? | | [SEP] to get to the $\to$ NEG & .667 & .108|.015 & .190|.030 & 0.0|.849 & .500|.030 & .418|.024 & .814|.894\\
%         \hline
%         \multirow{3}{*}{\sst} 
%         & the best $\to$ POS & .872 & .194 & .201 & .727 & .541 & .393 & .867\\
%         & a good $\to$ POS & .704 & .275 & .264 & .800 & .506 & .345 & .849\\
%         & in its $\to$ POS & .643 & .248 & .222 & .822 & .225 & .186 & .830\\
%         \hline
%         \multirow{3}{*}{\climate} 
%         & global warming [SEP] climate system $\to$ relevant & 1.0 & -& -& -& .287|.035 & .240|.024 & .852|.932\\
%         & global warming [SEP] intergovernmental panel $\to$ relevant & 1.0 & - & - & - & .278|.042 & .242|.029 & .849|.924\\
%         & global warming [SEP] the earth $\to$ relevant & 1.0 & - & - & - & .285|.038 & .246|.027 & .848|.922\\
%         \hline
%     \end{tabular}
%     \caption{Averaged rank scores over supporting instances of the rules with top coverage (cov). the scores with the superscript $^E$ are scores with \expred, while $^S$ indicates \lime. \textbf{Do the global rules agree with the local explanations of their applicable instances'?}}
%     \label{tab:faithful}
% \end{table*}



==> tables/rq2-agreement.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
        \hline
        dataset & c-rate\% & bias\% & F1 & decoy0 & nDCG0$^\text{E}$ & nDCG0$^\text{L}$ & decoy1 & nDCG1$^\text{E}$ & nDCG1$^\text{L}$ \\
        \hline
        \multirow{4}{*}{\movies} & 20 & 60 & .945/.934/.920/.945 & F/-/-/F & .782/----/----/.780 & .921/----/----/.913 & F/-/-/F & .709/----/----/---- & .917/----/----/.912\\
                                 & 20 & 90 & .889/.910/.915/.910 & T/F/F/- & .751/.768/.767/---- & .915/.920/.923/---- & T/F/T/- & .754/.612/.612/.696 & .901/.910/.914/---- \\
                                 & 80 & 60 & .904/.920/----/---- & F/F/F/F & .781/.790/.791/.785 & .914/.914/.920/.916 & T/T/T/F & .795/.683/.682/.696 & .914/.910/.907/.900 \\
                                 & 80 & 90 & .910/.910/.920/.910 & T/F/F/T & .783/.796/.794/.787 & .924/.925/.929/.928 & T/T/T/T & .670/.675/.674/.683 & .924/.920/.917/.923 \\
        \hline
        \multirow{5}{*}{\sst}    & 20 & 60 & .855/.864/.855/.855 &  &  &  &  &  & \\
                                 & 20 & 90 & .855/.846/.853/.857 &  &  &  &  &  & \\
                                 & 80 & 60 & .855/.857/.857/---- &  &  &  &  &  & \\
                                 & 80 & 90 & .850/.847/.840/---- &  &  &  &  &  & \\
        \hline
        \multirow{5}{*}{\multirc}& 20 & 60 &  &  &  &  &  &  & \\
                                 & 20 & 90 &  &  &  &  &  &  & \\
                                 & 80 & 60 &  &  &  &  &  &  & \\
                                 & 80 & 90 &  &  &  &  &  &  & \\
        \hline
        \multirow{5}{*}{\climate}& 20 & 60 &  &  &  &  &  &  & \\
                                 & 20 & 90 &  &  &  &  &  &  & \\
                                 & 80 & 60 &  &  &  &  &  &  & \\
                                 & 80 & 90 &  &  &  &  &  &  & \\
        \hline
    \end{tabular}
    \caption{Results of 100\% contamination $c$ and 60\% \~ 100\% $b$ on \movies~ \multirc~ and \sst~datasets. \Zijian{we'd better move this huge table in the appendix and leave the figures here only... 
    \textcolor{red}{this table will be put in appendix, replaced by \ref{fig:rq2}} in the paper.
    }
    }
    \label{tab:rq2}
\end{table*}


% \begin{table*}[h]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
%         \hline
%         dataset & c-rate\% & F1 & decoy0 & nDCG0$^\text{E}$ & nDCG0$^\text{S}$ & decoy1 & nDCG1$^\text{E}$ & nDCG1$^\text{S}$ \\
%         \hline
%         \multirow{5}{*}{\movies} & 10 & .905 & F & - & - & F & - & - \\
%                                  & 30 & .915 & F & - & - & F & - & - \\
%                                  & 50 & .868 & T & .859 & .769 & F & - & - \\
%                                  & 70 & .864 & T & .865 & .781 & T & .852 & .848\\
%                                  & 90 & .737 & T & .860 & .778* & T & .852 & .834*\\
%         \hline
%         \multirow{5}{*}{\multirc}  & 10  & & F & - & - & T & single missing & single missing\\
%                                  & 30  & & T & single missing & & T & single missing &\\
%                                  & 50  & & T & single missing & & T & single missing &\\
%                                  & 70  & & T & single missing & & T & single missing &\\
%                                  & 90  & & T & single missing & & T & single missing &\\
%         \hline
%         \multirow{5}{*}{\sst}  & 10  & & T & .557 & .739 & T & .503 & .470\\
%                                  & 30  & & T & .485 & .734 & T & .528 & .584\\
%                                  & 50  & & T & .527 & .692 & T & .528 & .666\\
%                                  & 70  & & T & .510 & .702 & F & - & -\\
%                                  & 90  & & T & .579 & .724 & F & - & - \\
%         \hline
%     \end{tabular}
%     \caption{Results of {10\%, 30\%, 50\%, 70\%, 90\%} contamination rate (c-rate, $c$) and 100\% bias ($b$) on \movies, \multirc, \sst~datasets.}
%     \label{tab:100a}
% \end{table*}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/rq2.png}
%     \caption{where -, + indicate low, high rate of contamination (c) or bias(b)}
%     \label{fig:rq2}
% \end{figure}

==> tables/rq3-agreement.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
        \hline
        dataset & rmv\% & F1 & target & nDCG$^\text{E}$ & nDCG$^\text{S}$ \\
        \hline
        \multirow{5}{*}{\movies}  & 20  & & & & \\
                                 & 40  & & & &\\
                                 & 60  & & & & \\
                                 & 80  & & & & \\
                                 & 100  & & & & \\
        \hline
        \multirow{5}{*}{\multirc}  & 20  & & & & \\
                                 & 40  & & & &\\
                                 & 60  & & & & \\
                                 & 80  & & & & \\
                                 & 100  & & & & \\
        \hline
        \multirow{5}{*}{\sst}  & 20  & & & & \\
                                 & 40  & & & &\\
                                 & 60  & & & & \\
                                 & 80  & & & & \\
                                 & 100  & & & & \\
        \hline
    \end{tabular}
    \caption{Results of {20\%, 40\%, 60\%, 80\%, 100\%} removal rate (rmv\%) on \sst dataset. \textcolor{red}{This table will be replaced by a line/bar chart on removal rate on different decoys.}}
    \label{tab:decoy_remove}
\end{table*}

==> tables/rq4-human-eval.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|l|l|l|}
        \hline
        dataset & model & rule & synthetic counterfactual\\
        \hline
        \multirow{5}{*}{\movies}  &  & & \\
                                 &  & & \\
                                 &  & & \\
                                 &  & & \\
                                 &   & & \\
        \hline
        \multirow{5}{*}{\multirc}  &  & & \\
                                 &  & &\\
                                 &  & & \\
                                 &  & & \\
                                 &   & & \\
        \hline
        \multirow{5}{*}{\sst}  &  & & \\
                                 & & & \\
                                 &  & &\\
                                 &  & & \\
                                 &  & &\\
        \hline
    \end{tabular}
    \caption{rq 4: 5 example rules on different language models that are evaluated to be right for wrong reasons by human annotators.To replace \ref{tab:faithful}, Fleiss' kappa will be in another plot.}
    \label{tab:human_evaluation}
\end{table*}
